Robust Transceiver Design for Full-Duplex Decode-and-Forward Relay-Assisted MIMO Systems

Robust transceiver design against unresolvable system uncertainties is of crucial importance for reliable communication. For instance, full-duplex communication suffers from such uncertainties when canceling the self-interference, since some residual self-interference (RSI) remains uncanceled due to imperfect channel knowledge. We consider a MIMO multi-hop system, where the source, the relay and the destination are equipped with multiple antennas. The considered decode-and-forward (DF) hybrid relay can operate in either half-duplex or full-duplex mode, and the mode changes adaptively depending on the RSI strength. We investigate a robust transceiver design problem, which maximizes the throughput rate of the worstcase RSI under the self-interference channel uncertainty bound constraint. The yielded problem turns out to be a non-convex optimization problem, where the non-convex objective is optimized over the cone of semidefinite matrices. Without loss of generality, we simplify the problem to the optimization over multiple scalar parameters using majorization theory. Furthermore, we propose an efficient algorithm to obtain a local optimal solution iteratively. Eventually, we obtain insights on the optimal antenna allocation at the relay input-frontend and output-frontend, for relay reception and transmission, respectively. Interestingly, given a number of antennas at the relay, the robustness improves if more antennas are allocated to reception than to transmission.

==> main10.tex <==
\(pdf)latex mypaper
\bibtex mypaper

==> zayeat.tex <==
%5The objective of this problem is an affine function. Moreover, the constraints~\eqref{P:FDd:ConsB} and~\eqref{P:FDb:ConsA}-\eqref{P:FDb:ConsC} are convex constraints. However, the constraint~\eqref{P:FDd:ConsA} is a non-convex constraint, since the RHS is not necessarily a concave function of the optimization parameters. Hence, the problem is a non-convex optimization problem. Furthermore, notice that the minimum of the objective function w.r.t. $\boldsymbol{\sigma}_{\mathrm{r}}$ is maximized w.r.t. $R,\boldsymbol{\gamma}_\mathrm{s},\boldsymbol{\gamma}_\mathrm{r}$. Next, we propose an efficient algorithm for obtaining a stationary point.
%
%
\begin{figure*}
\right
\begin{minipage}{0.2\textwidth}
%{0.2\textwidth}
\subfigure[$\{M,K_\mathrm{r}+K_\mathrm{t},N\}=\{4,10,4\}$]{
\tikzset{every picture/.style={scale=.8}, every node/.style={scale=0.8}}%
\input{asli}
\label{fig:HdVsFdB}
}
\end{minipage}
\quad\quad\quad\quad\quad\quad\quad
%\begin{minipage}{0.2\textwidth}
%\subfigure[$\{M,K_\mathrm{r}\}=\{10,15\}$]{
%\tikzset{every picture/.style={scale=0}, every node/.style={scale=0.7}}%
%\input{myfile1}
%\label{fig:myfile1}
%}
%\end{minipage}
%\\
\begin{minipage}{0.2\textwidth}
%{0.2\textwidth}
\subfigure[$\{M,K_\mathrm{r}+K_\mathrm{t},N\}=\{10,24,10\}$]{
\tikzset{every picture/.style={scale=.8}, every node/.style={scale=0.8}}%
\input{myfile}
\label{fig:HdVsFdE}
}
\end{minipage}
\caption{The transmit power budget at the source and the relay are assumed to be equal, i.e., $P_\mathrm{s}=P_\mathrm
r=P=5$.}
\label{fig:HdVsFdBD}
\end{figure*}

%\subsection{Optimization Algorithm}
%The proposed algorithm is based on the following intuitions,
%\begin{enumerate}
%\item given optimal $\bar{\sigma}_{1_i},\ \forall i,$ (genie-aided), the problem is solved by the water-filling algorithm.
%\item by allocating more power to the $i$-th stream at the relay, the worst-case SI channel has more power for that stream as well.
%\item the rate of the $i$-th stream of the source-relay link is reduced as $\gamma_{\mathrm{r}_i}$ and/or $\sigma_{\mathrm{r}_i}$ increase.
%\item at the relay, transmitting with less power than the available power budget, reduces the throughput rate of the relay-destination link, but increases the throughput rate of the source-relay link.
%\end{enumerate}

%The algorithm is based on successive water-filling procedures with are iterated. This procedure is explained for the $l$-th iteration as follows
%\begin{enumerate}[(I)]
%\item the relay-destination rate is maximized by allocating more power to better channels, and obtaining a water level $\tau^{(l)}_r$, which satisfies the power budget $P^{(l)}_\mathrm{r}\leq P_\mathrm{r}$,
%\item the worst-case SI channel is the one that interferes the strong data-streams (data-streams with high power) received at the relay more than the interference on the weak streams. This is realized by water-filling, and obtaining a water level $\tau^{(l)}_\mathrm{SI}$ that satisfies the water level $T$.
%\item having the solutions from (I) and (II), the optimal power allocation at the source is fulfilled by water-filling with water level $\tau^{(l)}_\mathrm{s}$, which satisfies the power constraint $P_\mathrm{s}$,
%\item having the solutions from (I), (II) and (III), we compute the achievable source-relay and relay-destination rates, i.e., $R^{(l)}_\mathrm{sr}$ and $R^{(l)}_\mathrm{rd}$. If $|R^{(l)}_\mathrm{rd}-R^{(l)}_\mathrm{sr}|$ is still large, we perform step (I) with a power budget less than $P^{(l)}_\mathrm{r}$.
%\end{enumerate}
%We present the algorithm pseudo-code in details in Algorithm 1. It is crucial to note that the parameters $\boldsymbol{\sigma}_\mathrm{r}$ and $\boldsymbol{\gamma}_\mathrm{s}$ play a non-collaborative game in the inner-loop for a fixed strategy $\boldsymbol{\gamma}_\mathrm{r}$ which is updated in the outer-loop.
